Denoised MDPs: Learning World Models Better Than the World Itself

The ability to separate signal from noise, and reason with clean abstractions, is critical to intelligence. With this ability, humans can efficiently perform real world tasks without considering all possible nuisance factors.How can artificial agents do the same? What kind of information can agents safely discard as noises? In this work, we categorize information out in the wild into four types based on controllability and relation with reward, and formulate useful information as that which is both controllable and reward-relevant. This framework clarifies the kinds information removed by various prior work on representation learning in reinforcement learning (RL), and leads to our proposed approach of learning a Denoised MDP that explicitly factors out certain noise distractors. Extensive experiments on variants of DeepMind Control Suite and RoboDesk demonstrate superior performance of our denoised world model over using raw observations alone, and over prior works, across policy optimization control tasks as well as the non-control task of joint position regression.

==> figtext/02_real_world_information/mdp_transition_grid_xonly.tex <==
%auto-ignore
%!TEX root = ../../main.tex

\begin{figure*}[ht]
    % \vspace{0.01cm}
    % \vspace{-19pt}
    \vspace{5pt}
    \centering
    \begin{subfigure}[t]{4.9cm}
        \centering
        \scalebox{0.9}{
        \hspace{-0.1cm}\begin{tikzpicture}[bayes_net, node distance = 0.5cm, every node/.style={inner sep=0, minimum size = 0.9cm}]
            \node[main_node] (s) {$s$};
            \node[draw=none] (dummy) [below=-0.82cm of s] {};
            \node[main_node] (sp) [right = 0.4cm of s] {$s'$};
            \node[main_node, draw=none, text opacity=0] (aheightholder) [above right = 3.85cm and 0.1cm of s] {$a$};
            \node[main_node] (a) [above right = 1.15cm and -0.175cm of s] {$a$};
            \node[main_node] (r) [above right = 1.15cm and -0.4cm of sp] {$r$};

            \node[minimum size = 1.075cm, draw=none, inner sep=0, label={[scale=1.2]center:$s$}] (cbr) [above right = -0.75cm and 1.1cm  of sp] {};
            \node[minimum size = 1.075cm, draw=none, label={[scale=1.2]center:$s$}] (cbrb) [right = -0.03cm of cbr] {};
            \node[minimum size = 1.075cm, draw=none, label={[scale=1.2]center:$s$}] (cr) [above = -0.03cm of cbr] {};
            \node[minimum size = 1.075cm, draw=none, label={[scale=1.2]center:$s$}] (crb) [right = -0.03cm of cr] {};
            \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{Ctrl}}] () [left = 0cm of cr] {};
            \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{\textoverline{Ctrl}}}] () [left = 0cm of cbr] {};
            \node[draw=none, minimum height=.33cm, label={[scale=0.9]center:\textbf{Rew}}] () [above = 0cm of cr] {};
            \node[draw=none, minimum height=.4cm, label={[scale=0.9]center:\textbf{\textoverline{Rew}}}] () [above = 0cm of crb] {};

            \tikzset{myptr/.style={decoration={markings,mark=at position 1 with %
                {\arrow[scale=0.825,>=stealth']{>}}},postaction={decorate}}}
            \path[]
            (s) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (sp)
            (a) edge[-, myptr, line width=1.2pt] [right] node [below=3pt] {} (sp)
            (sp) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (r)
            ;
        \end{tikzpicture}
        }\vspace{-5pt}%
        \caption{Transition without useful structure. $s$ may contain any type of information.}\label{fig:mdp-grid-regular}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{5.6cm}
        \centering
        \scalebox{0.9}{
        \hspace{-0.1cm}\begin{tikzpicture}[bayes_net, node distance = 0.5cm, every node/.style={inner sep=0, minimum size = 0.9cm}]
            \node[main_node] (s) {$s$};
            \node[main_node, color=MyColorYRB] (y) [above = 0.45cm of s] {$y_{\overbar{R}}$};
            \node[main_node, color=MyColorYR] (yR) [above = 0.225cm of y] {$y_R$};
            \node[main_node, color=MyColorX] (x) [above = 0.225cm of yR] {$x$};
            \node[main_node] (sp) [right = 0.8cm of s] {$s'$};
            \node[main_node, color=MyColorX] (xp) [right = 0.8cm of x] {$x'$};
            \node[main_node, color=MyColorYR] (yRp) [right = 0.8cm of yR] {$y_R'$};
            \node[main_node, color=MyColorX] (rx) [right = 0.385cm of xp] {$r_x$};
            \node[main_node, color=MyColorYR] (ry) [right = 0.385cm of yRp] {$r_y$};
            \node[main_node, color=MyColorYRB] (yp) [right = 0.8cm of y] {$y'_{\overbar{R}}$};
            \node[main_node] (a) [above right = 4cm and 0.1cm of s] {$a$};
            \node[minimum width=0.335cm, minimum height=0.75cm, draw] (plus) [above right = -0.15cm and 0.35cm of ry] {$+$};
            \node[main_node] (r) [right = 0.25cm of plus] {$r$};

            % \begin{pgfinterruptboundingbox}
            % \node [draw=none, minimum width=12cm, minimum height=3cm] (test) [above right = -0.9cm and -0.9cm of x] {test};
            % \end{pgfinterruptboundingbox}

            \tikzset{myptr/.style={decoration={markings,mark=at position 1 with %
                {\arrow[scale=0.825,>=stealth']{>}}},postaction={decorate}}}
            \path[]
            (x) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (xp)
            (xp) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (rx)
            (rx.345) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (plus)
            (a) edge[-, myptr, line width=1.2pt] [right] node [below=3pt] {} (xp)
            (y) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (yp)
            (yR) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (yRp)
            (yRp) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (ry)
            (ry.15) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (plus)
            (plus) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (r)
            (y) edge[-, myptr, line width=1.2pt, shorten <= 0.13cm] [right] node [midway, above=3pt] {} (s)
            (yp) edge[-, myptr, line width=1.2pt, shorten <= 0.13cm] [right] node [midway, above=3pt] {} (sp);

            % \node[minimum size = 1cm, draw] (cbr) [above right = -0.75cm and 1.3cm  of sp] {\color{red}$y_R$};
            % \node[minimum size = 1cm, draw] (cbrb) [right = -0.03cm of cbr] {\cyrb};
            % \node[minimum size = 1cm, draw] (cr) [above = -0.03cm of cbr] {\cx};
            % \node[minimum size = 1cm, draw] (crb) [right = -0.03cm of cr] {\cx};

            \node[minimum size = 1.075cm, draw] (cbr) [above right = -0.75cm and 1.3cm  of sp] {};
            \node[minimum size = 1.075cm, draw] (cbrb) [right = -0.03cm of cbr] {};
            \node[minimum size = 1.075cm, draw] (cr) [above = -0.03cm of cbr] {};
            \node[minimum size = 1.075cm, draw] (crb) [right = -0.03cm of cr] {};

            \node[] (cbrx) [above = -0.875cm of cbr] {\cx};
            \node[] (crx) [above = -0.875cm of cr] {\cx};
            \node[] (crbx) [above = -0.875cm of crb] {\cx};
            \node[] (cbrbx) [above = -0.875cm of cbrb] {\cx};

            \node[text opacity=0] (cbry) at ([shift={(-0.215,-0.335)}]cbrx) {\cyrb};
            \node[text opacity=0] (cry) at ([shift={(-0.215,-0.335)}]crx) {\cyrb};
            \node[text opacity=0] (crby) at ([shift={(-0.215,-0.335)}]crbx) {\cyrb};
            \node[] (cbrby) at ([shift={(-0.215,-0.335)}]cbrbx) {\cyrb};

            \node[] (cbryr) at ([shift={(0.275,-0.319)}]cbrx) {\cyr};
            \node[text opacity=0] (cryr) at ([shift={(0.275,-0.319)}]crx) {\cyr};
            \node[text opacity=0] (crbyr) at ([shift={(0.275,-0.319)}]crbx) {\cyr};
            \node[] (cbrbyr) at ([shift={(0.275,-0.319)}]cbrbx) {\cyr};

            \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{Ctrl}}] () [left = 0cm of cr] {};
            \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{\textoverline{Ctrl}}}] () [left = 0cm of cbr] {};
            \node[draw=none, minimum height=.33cm, label={[scale=0.9]center:\textbf{Rew}}] () [above = 0cm of cr] {};
            \node[draw=none, minimum height=.4cm, label={[scale=0.9]center:\textbf{\textoverline{Rew}}}] () [above = 0cm of crb] {};

            \begin{scope}[on background layer]
                \draw[fill=black, fill opacity=0.08, color=black, -, dashed, shorten >= 0pt] \convexpath{x,y}{0.575cm};
                \draw[fill=black, fill opacity=0.08, color=black, -, dashed, shorten >= 0pt] \convexpath{xp,yp}{0.575cm};
            \end{scope}
        \end{tikzpicture}%
        }\vspace{-5pt}%
        % \caption{MDP transition that separates controllable {\cx}, uncontrollable and unrelated to reward {\cyrb}, and uncontrollable but  related to reward {\color{red}$y_R$}.}%
        \caption{Transition that factorizes out \nctrl information in {\cyrb} and \cyr. %Our Denoised MDP (see \Cref{sec:denoise}) is built upon this factorization.
        }%
        \label{fig:mdp-grid-xy}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{5.6cm}
        \centering
        \scalebox{0.9}{
        \hspace{-0.1cm}\begin{tikzpicture}[bayes_net, node distance = 0.5cm, every node/.style={inner sep=0, minimum size = 0.9cm, draw=none}]
            \node[main_node] (s) {$s$};
            \node[main_node, color=MyColorZ] (z) [above = 0.45cm of s] {$z$};
            \node[main_node, color=MyColorY,draw=none,text opacity=0] (y) [above = 0.225cm of z] {$y$};
            \node[main_node, color=MyColorX,draw=none,text opacity=0] (x) [above = 0.225cm of y] {$x$};
            \node[main_node] (sp) [right = 0.8cm of s] {$s'$};
            \node[main_node, color=MyColorX] (xp) [right = 0.8cm of x] {$x'$};
            \node[main_node, color=MyColorY] (yp) [right = 0.8cm of y] {$y'$};
            \node[main_node, color=MyColorX,draw=none,text opacity=0] (rx) [right = 0.385cm of xp] {$r_x$};
            \node[main_node, color=MyColorY,draw=none,text opacity=0] (ry) [right = 0.385cm of yp] {$r_y$};
            \node[main_node, color=MyColorZ] (zp) [right = 0.8cm of z] {$z'$};
            \node[main_node] (a) [above right = 4cm and 0.1cm of s] {$a$};
            \node[minimum width=0.335cm, minimum height=0.75cm, draw] (plus) [above right = -0.15cm and 0.35cm of ry] {$+$};
            \node[main_node] (r) [right = 0.25cm of plus] {$r$};

            \tikzset{myptr/.style={decoration={markings,mark=at position 0.99999 with %
                {\arrow[scale=0.825,>=stealth']{>}}},postaction={decorate}}}
            \path[]
            % (x) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (xp)
            % (xp) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (rx)
            (rx.345) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (plus)
            % (a) edge[-, myptr, line width=1.2pt] [right] node [below=3pt] {} (xp)
            % (y) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (yp)
            % (yp) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (ry)
            (ry.15) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (plus)
            (plus) edge[-, myptr, line width=1.2pt] [right] node [left=3pt] {} (r)
            (a) edge[-, myptr, line width=1.2pt, bend right=20] [right] node [midway, above=3pt] {} (zp)
            (z) edge[-, myptr, line width=1.2pt] [right] node [midway, above=3pt] {} (zp)
            (yp) edge[-, myptr, line width=1.2pt] [right] node [midway, above=3pt] {} (zp)
            (z) edge[-, myptr, line width=1.2pt, shorten <= 0.13cm] [right] node [midway, above=3pt] {} (s)
            (xp) edge[-, myptr, line width=1.2pt, bend left=35] [left] node [midway, above=3pt] {} (zp)
            (zp) edge[-, myptr, line width=1.2pt, shorten <= 0.13cm] [right] node [midway, above=3pt] {} (sp);

            % % \node[minimum size = 0.8cm, draw] (cbr) [above right = -0.75cm and 1.4cm  of sp] {\cy};
            % % \node[minimum size = 0.8cm, draw] (cbrb) [right = -0.03cm of cbr] {\cy};
            % % \node[minimum size = 0.8cm, draw] (cr) [above = -0.03cm of cbr] {\cx};
            % % \node[minimum size = 0.8cm, draw] (crb) [right = -0.03cm of cr] {\cz};

            % \node[minimum size = 1.075cm, draw] (cbr) [above right = -0.75cm and 1.3cm  of sp] {};
            % \node[minimum size = 1.075cm, draw] (cbrb) [right = -0.03cm of cbr] {};
            % \node[minimum size = 1.075cm, draw] (cr) [above = -0.03cm of cbr] {};
            % \node[minimum size = 1.075cm, draw] (crb) [right = -0.03cm of cr] {};

            % \node[] (cbrx) [above = -0.875cm of cbr] {\cx};
            % \node[] (crx) [above = -0.875cm of cr] {\cx};
            % \node[] (crbx) [above = -0.875cm of crb] {\cx};
            % \node[] (cbrbx) [above = -0.875cm of cbrb] {\cx};

            % \node[] (cbry) at ([shift={(-0.2,-0.33)}]cbrx) {\cy};
            % \node[text opacity=0] (cry) at ([shift={(-0.2,-0.33)}]crx) {\cy};
            % \node[text opacity=0] (crby) at ([shift={(-0.2,-0.33)}]crbx) {\cy};
            % \node[] (cbrby) at ([shift={(-0.2,-0.33)}]cbrbx) {\cy};

            % \node[text opacity=0] (cbrz) at ([shift={(0.215,-0.3075)}]cbrx) {\cz};
            % \node[text opacity=0] (crz) at ([shift={(0.215,-0.3075)}]crx) {\cz};
            % \node[] (crbz) at ([shift={(0.215,-0.3075)}]crbx) {\cz};
            % \node[] (cbrbz) at ([shift={(0.215,-0.3075)}]cbrbx) {\cz};

            % \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{Ctrl}}] () [left = 0cm of cr] {};
            % \node[draw=none, minimum width=.7cm, label={[scale=0.9]center:\textbf{\textoverline{Ctrl}}}] () [left = 0cm of cbr] {};
            % \node[draw=none, minimum height=.33cm, label={[scale=0.9]center:\textbf{Rew}}] () [above = 0cm of cr] {};
            % \node[draw=none, minimum height=.4cm, label={[scale=0.9]center:\textbf{\textoverline{Rew}}}] () [above = 0cm of crb] {};

            % \begin{scope}[on background layer]
            %     \draw[fill=black, fill opacity=0.08, color=black, -, dashed, shorten >= 0pt] \convexpath{x,z}{0.575cm};
            %     \draw[fill=black, fill opacity=0.08, color=black, -, dashed, shorten >= 0pt] \convexpath{xp,zp}{0.575cm};
            % \end{scope}
        \end{tikzpicture}
        }\vspace{-5pt}%
        % \caption{MDP transition that separates uncontrollable {\cy}, controllable but unrelated to reward {\cz} and controllable and related to reward {\cx}.}%
        \caption{Transition that factorizes out \nctrl $\cy$ and \nrewrel $\cz$.}%
        \label{fig:mdp-grid-xyz}
    \end{subfigure}\vspace{-6.5pt}%
    \caption{MDP transition structures consisting of dynamics and reward functions. Unlike the regular structure of \textbf{(a)}, \textbf{(b,~c)} factorized (yet still general) structures  inherently separate information into \ctrl (\textbf{Ctrl}) versus \nctrl (\textbf{\textoverline{Ctrl}}), and \rewrel (\textbf{Rew}) versus \nrewrel (\textbf{\textoverline{Rew}}). Presence of a variable in a cell means \emph{possible} containing of respective information. \Eg, in \textbf{(c)}, $\cz$ can only contain \nrewrel information\hide{, regardless of controllability}. In \textbf{(b,~c)}, the $\cx$ dynamics form an MDP with less noise and sufficient for optimal planning. Our Denoised MDP (see \Cref{sec:denoise}) is based on these two factorizations.}\label{fig:mdp-transition-grid}
    \vspace{-4.5pt}
\end{figure*}%


==> figtext/05_experiments/dmc_aggregated_rew_wide.tex <==
%auto-ignore

\vspace{-9pt}%
\hspace*{-1.2em}%
\centering%
\resizebox{
  0.78\width
}{!}{%
\small%
\centering%
\newlength{\digitl}\settowidth{\digitl}{1}
\newlength{\basel}\settowidth{\basel}{.1}
\newlength{\tinydigitl}\settowidth{\tinydigitl}{\tiny1}
\newlength{\tinybasel}\settowidth{\tinybasel}{\tiny.1}
\newcommand{\mround}[3][3]{\makebox[\basel+3\digitl][r]{\round{#2}{1}}~{\tiny\textpm~\makebox[\tinybasel+#1\tinydigitl][r]{\round{#3}{1}}}}%
\newcommand{\mroundprec}[1]{\round{#1}{2}\%\xspace}%
\newcommand{\bftab}{\fontseries{b}\selectfont}%
\renewcommand{\arraystretch}{1.3}%
\renewcommand{\arraystretch}{1.28}%
\setlength{\tabcolsep}{0.3em} % for the horizontal padding
\setlength\extrarowheight{1pt}
\begin{tabular}{ccccccccc@{\hskip 1.6em}cc}
    \toprule
    \multirow{2}{*}[-3pt]{Noise Variant}
    &  \multicolumn{3}{c}{\textbf{Policy Learning:} Backprop via Dynamics}
    &  \multicolumn{3}{c}{\textbf{Policy Learning:} SAC (Latent-Space)}
    & \multirow{2}{*}[-3pt]{DBC}
    & \multirow{2}{*}[-3pt]{\shortstack{PI-SAC\\[0.2ex](No Aug.)}}
    & \color{gray}\multirow{2}{*}[-3pt]{\shortstack{CURL\\[0.22ex](Use Aug.)}}
    & \color{gray}\multirow{2}{*}[-3pt]{\shortstack{State-Space SAC\\[-0.19ex](Upper Bound)}}
    \\
    \cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}

    & Denoised MDP
    & TIA
    & Dreamer
    & Denoised MDP
    & TIA
    & Dreamer
    &
    &
    &
    &
    \\
    \midrule

    \textbf{Noiseless}
    & \mround{801.4036376953126}{96.5631806020146}%\mround{827.388314819336}{70.42618595462613}
    & \mround{769.6890177408854}{97.07365040080172}
    & \bftab\mround{848.5710754394531}{137.1229304081701}
    & \bftab\mround{587.0703776041667}{98.65461107426525}%\mround{638.9795135498047}{66.17454307411509}
    & \mround{480.2342773437501}{125.52896905820866}
    & \mround{575.4169545491537}{146.1595737300942}
    & \mround[2]{297.3831787109375}{72.5317611694336}
    & \mround[2]{246.4079319000244}{56.6048894290624}
    & \color{gray}\mround{417.27490234375}{183.1774444580078}
    & \color{gray}\mround{910.32275390625}{28.20912742614746}
    \\
    
    \textbf{Video Background}
    & \bftab\mround{597.7299418131511}{117.80636716375385}
    & \mround{407.12691319783534}{225.361746235247}
    & \mround{227.78392486572264}{102.74045289489862}
    & \mround{309.84704717000324}{153.0209530309676}
    & \bftab\mround{318.1289639790853}{123.65134941187614}
    & \mround{188.7033597310384}{78.19801845086053}
    & \mround[2]{187.9536895751953}{67.35724639892578}
    & \mround[2]{131.7182393391927}{20.061926016930414}
    & \color{gray}\mround{477.962562790126}{113.45766739421701}
    & \color{gray}\mround{910.32275390625}{28.20912742614746}
    \\
    
    \textbf{Video Background + Noisy Sensor}
    & \bftab\mround{563.1350830078126}{142.9780084788406}
    & \mround{261.16744333902994}{200.36596272685793}
    & \mround{212.40484008789062}{89.70869711827993}
    & \bftab\mround{288.17919921875}{123.35275437438976}
    & \mround{197.2980753580729}{124.17133774817682}
    & \mround{218.22257232666016}{58.14234620401891}
    & \mround[2]{79.92886352539062}{35.982017517089844}
    & \mround[2]{152.49693603515627}{12.565573870135873}
    & \color{gray}\mround{354.32098393849896}{119.85382267836293}
    & \color{gray}\mround{919.7915649414062}{100.7192153930664}
    \\
    
    \textbf{Video Background + Camera Jittering}
    & \bftab\mround{254.08687286376957}{114.17497499531767}
    & \mround{151.69740829467773}{160.50280245308895}
    & \mround{98.55416285196941}{27.744005563777023}
    & \bftab\mround{186.8494852701823}{47.67715965353988}
    & \mround{126.46733729044597}{125.60276425491514}
    & \mround{105.15849736531577}{33.79692949925169}
    & \mround[2]{68.00225067138672}{38.433292388916016}
    & \mround[2]{91.62684427897136}{7.587171023260147}
    & \bftab\color{gray}\mround{390.4128860804934}{64.91543681192832}
    & \color{gray}\mround{910.32275390625}{28.20912742614746}
    \\
    \bottomrule
\end{tabular}%
}%
\vspace{-5pt}%
\caption{\new{DMC policy optimization results. For each variant, we aggregate performance across three tasks (Cheetah Run, Walker Walk, Reacher Easy) by averaging. Denoised MDP performs well across all four variants with distinct noise types. \textbf{Bold numbers} show the best model-learning result for specific policy learning choices, or the best overall result. On \textbf{Camera Jittering}, Denoised MDP greatly outperforms all other methods except for CURL, which potentially benefits from its specific data augmentation choice (random crop) on this task, and can be seen as using extra information (\ie, knowing the noise distractor form). In fact, Denoised MDP is the only method that consistently performs well across all tasks and noise variants, which can be seen from the full results in the appendix.}}\label{tbl:dmc-agg-rew}
\vspace{-3pt}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> text/05_experiments_old.tex <==
%auto-ignore
%!TEX root = ../main.tex
\input{figtext/05_experiments/dmc_recon}
\input{figtext/05_experiments/dmc_rew}

\section{Experiments}\label{sec:expr}

In this section, we contrast our method with existing approaches on environments with image observations and many distinct types of noisy distractors. Our experiments are designed to include a variety of noise distractors and to confirm our analysis on various methods in \Cref{sec:grid-existing}.

In \Cref{sec:dmc},  we evaluate on the popular DeepMind Control (DMC) Suite \citep{tunyasuvunakool2020dm_control}, including the natural video background distractor established by \citeauthor{zhang2020learning} and other novel noise types, revealing drawbacks of several baselines. In \Cref{sec:robodesk}, we augment the \robodesk environment \citep{kannan2021robodesk} with naturally occurring noises such as light flickering and camera jittering, and demonstrate that our learned model is beneficial for both policy learning and non-control tasks.

For comparison, we consider not only model-based RL methods, but also model-free algorithms and general contrastive representation learning approaches, when the task is suited: \begin{itemize}
    \item \textbf{Denoised MDP}: our method described in \Cref{sec:denoise}.
    \item \textbf{Dreamer \citep{hafner2019dream}}: a well-established model-based method (see \Cref{sec:grid-existing}).
    \item \textbf{Task Informed Abstractions (TIA) \citep{fu2021learning}}: a recent model-based method with a complex structure for handling distractors and signals composed via masking (see \Cref{sec:grid-existing}).
    \item \textbf{Deep Bisimulation for Control (DBC) \citep{zhang2020learning}}: a model-free method that optimizes policies on top of a learned on-policy bisimulation metric embedding (see \Cref{sec:grid-existing}).
    \item \textbf{Stochastic Actor-Critic (SAC) \citep{haarnoja2018soft} on true state-space}: a model-free algorithm using the ``optimal'' feature space specific to each environment (rather than the image observations). This presents a rough ``upper bound'' reference.
    \item \textbf{Contrastive image representation learning}: for non-control tasks, we compare with image encoders learned with a general image representation learning method, the contrastive loss from \citet{wang2020hypersphere}.
\end{itemize}
The three model-learning methods can be used in combination with any policy optimization algorithm. For a more complete view of how well each model is suited for control, we consider two policy learning procedures, and compare the models under each: (1) backpropagating via the learned dynamics and (2) SAC on the learned latent space (which roughly recovers SLAC \citep{lee2019stochastic}).

All results are aggregated from 5 runs with different random seeds. Please refer to the appendix for experiment details, hyperparameter studies, and additional  results.

For Denoised MDP, we use the \Cref{fig:mdp-grid-xy} variant. Empirically, the \Cref{fig:mdp-grid-xyz} variant leads to longer training and often inferior performance (likely due to having to optimize extra components and fit a more complex model). The appendix provides an comparison between them.

\subsection{DeepMind Control Suite (DMC)}\label{sec:dmc}

\paragraph{Environment variants.} To evaluate a diverse set of noisy distractors, we consider four variants for any particular DMC task with image observation (see \Cref{fig:dmc-recon} top row): \begin{itemize}
    \item \textbf{Noiseless}: Original environment without distractors.
    \item \textbf{Video Background}: Replacing noiseless background with natural videos \citep{zhang2020learning}, a distractor that is \emph{\nctrl} and \emph{\nrewrel} ($\overbar{\textbf{Ctrl}}\&\overbar{\textbf{Rew}}$).
    \item \textbf{Video Background + Sensor Noise}: In addition to \textbf{Video Background}, modeling imperfect sensors as sensitive to the intensity of a background patch, which \emph{affects the reward} but is \emph{\nctrl} ($\overbar{\textbf{Ctrl}}\&\textbf{Rew}$).
    \item \textbf{Video Background + Camera Jittering}: In addition to \textbf{Video Background}, the observation image undergoes a smooth random jittering, which is also both  \emph{\nctrl} and \emph{\nrewrel} ($\overbar{\textbf{Ctrl}}\&\overbar{\textbf{Rew}}$).
\end{itemize}

\paragraph{Denoised MDP cleanly separates signals from many types of noises.} \Cref{fig:dmc-recon} visualizes models learned by various methods. For TIA and Denoised MDP, the \textsf{Signal} and \textsf{Noise} rows also show what the models capture as signals versus noises. Importantly, (1) \emph{components that change in these images} are what the model considers as signal or noise (2) image clarity doesn't correspond to better feature, due to the inherent different ways TIA and Denoised MDP provides these images. Instead, our focus is on the different information categorization.
As analyzed in \Cref{sec:grid-existing}, TIA considers observations as a mask-composition of a signal image and noise image, which is independent of rewards. It thus can separate out simple distractors that can be modelled this way (Walker Walk with \textbf{only Video Background}). However, it fails on \textbf{Video Background} variant of Reacher Easy, where the reward is given by the distance between the robot and a randomly-located ball. TIA encourages the noise latent to be independent of reward, but does not prevent it from capturing the \ctrl agent. Consistent with our analysis, the TIA structure (discussed in \Cref{sec:grid-existing}) also struggles on distractors that can not be represented this way, such as \textbf{Sensor Noise} (noise that affects reward) and \textbf{Camera Jittering} (noise that may not be modelled via masking). In these cases, it either tries to model everything in the signal component, or learns a bad model (\eg, wrong agent position in last column). In comparison, over all variants Denoised MDPs learn signal components containing only moving agents and unaffected by the noisy background and camera jittering, and noise components with static agents and only moving background and jittering, indicating a successful  separation. With a much simpler structure than TIA, Denoised MDP can better identify and remove many more noise types.

% Denoised MDPs has a much simpler structure but almost always cleanly separates noise and signals over all variants. In \Cref{fig:dmc-recon}, Denoised MDPs learn signal components containing only moving agents and unaffected by the noisy background and camera jittering, and noise components with static agents and only moving background and jittering

\paragraph{Denoised MDP helps policy learning under noises. } Better denoised model indeed leads to better learned policies. In \Cref{fig:dmc-rew}, we compare policies learned from various model-based and model-free approaches. While many baselines can learn well under noiseless settings (and some noisy background settings for TIA), only Denoised MDPs consistently enables finding good policies over all settings, and for both policy optimization algorithms, likely due to its consistent denoising results over these environments (see \Cref{fig:dmc-recon}). Dreamer and TIA both struggle on environments where they are unable to learn clean features (\eg, \textbf{Video Background} for Dreamer, and \textbf{Noisy Sensor} for TIA). DBC is also consistently the worst method on \textbf{Noisy Sensor} settings, consistent with our analysis in \Cref{sec:grid-existing} that it can not handle \rewrel noises.

\paragraph{Learning in clean denoised world model is better than learning in the real world. } We highlight that SAC learning is possible on good clean learned models (in \Cref{fig:dmc-rew}), while it is known to fail on the original environment of image observations \citep{kostrikov2020image,yarats2021mastering}. This qualitative difference suggest the benefits of learning on top of a model, rather than the real world. The performance difference between Denoised MDP and other models further emphasizes that denoising is crucial, in addition to potential benefits of using lower-dimensional latent spaces.

\subsection{\robodesk with More Natural Noisy Distractors} \label{sec:robodesk}

% Moving beyond the artificial noises in DMC, w
We explore a more sophisticated simulated environment, and augment it with a variety of more natural noise distractors. In our \robodesk variant \citep{kannan2021robodesk}, the agent controls a robotic arm placed in front of a desk and a TV, and is tasked to push down the green button on the desk, which turns on a small green light and makes the TV display have a green hue. The intensity of the TV image's green channel is given to the agent as part of their reward. Additionally, the environment contains other noisy distractors, including moveable blocks on the desk ($\textbf{Ctrl}\&\overbar{\textbf{Rew}}$), flickering environment light and camera jittering  ($\overbar{\textbf{Ctrl}}\&\overbar{\textbf{Rew}}$), natural RGB video playing on the TV  ($\overbar{\textbf{Ctrl}}\&\textbf{Rew}$), and noisy button sensors  ($\overbar{\textbf{Ctrl}}\&\textbf{Rew}$).

\input{figtext/05_experiments/robodesk_joint_pos}
\input{figtext/05_experiments/robodesk_recon}
\input{figtext/05_experiments/robodesk_rew}

\paragraph{Only Denoised MDP learns a clean model, which enables better policy learning.} In \Cref{fig:robo-recon}, TIA fails to separate any noise since due to its limitation to only \nrewrel noises and can be represented via masking. Denoised MDP, however, learns a signal component that only correspond to relevant information including robot arm state, ``green-ness'' of TV image. It is completely unaffected by any camera, lighting, or TV semantic content changes, which are exclusively captured by the noise component. Such clean learned models are useful for control, as confirmed by \Cref{fig:robo-rew} where backpropagating via dynamics learns better policies from Denoised MDPs.


% \paragraph{Denoised MDP enables better policy learning using backpropagating via dynamics.} \Cref{fig:robo-rew} reconfirms that better and clean model is useful for policy learning. Additionally,
% shows superior policies learned on Denoised MDP from backpropagating via dynamics. With latent-space SAC, there is no clear separation.

% \paragraph{Different noise amounts imply different optimal regularization ammount.} Here, as we zoom out/in the viewing camera, more/less TV pixels are included in the observation. This gives us a way to roughly change the level of noises present in the observation, which may require different amounts of regularization.  \Cref{fig:robo-lon} confirms this hypothesis and shows that greater noises require a stronger regularizer (\ie, smaller $\beta$) for optimal policy learning.

\subsubsection{Robot Arm Joint Position Regression}\label{sec:robo-joint-regression}


Moving beyond control tasks, we evaluate the learned world models' representations on a supervised task--- regressing the robot arm joint position. Using encoders trained with various methods, we finetune on a labeled dataset consisting pairs of image observations and joint positions, and measure mean squared error (MSE) on a heldout test set. In addition to RL methods, we compare image contrastive learning on the same amount of data.  Denoised MDP representation leads to best converged solution across a wide range of training set sizes (\Cref{sub@fig:robo-joint-pos-final}), achieves faster training (\Cref{fig:robo-joint-pos-train-curve-small,sub@fig:robo-joint-pos-train-curve-large}), and  avoids overfitting with small training sets (\Cref{fig:robo-joint-pos-train-curve-small}). Indeed, clean denoised world models are beneficial beyond control tasks.

% \fixme{Paragraph discussing results: better converged point, faster learning}


% 2. more realistic noises in robodesk

% 2a. policy learning

% + reward plot

% + viz recon. see how things change as task changes

% + viz opt beta as LoN changes

% 2b. joint position regression

% + final mse

% + speed
